XplainLLM: A Knowledge-Augmented Dataset for Reliable Grounded Explanations in LLMs

Large Language Models (LLMs) have achieved remarkable success in natural language tasks, yet understanding their reasoning processes remains a significant challenge. We address this by introducing XplainLLM, a dataset accompanying an explanation framework designed to enhance LLM transparency and reliability. Our dataset comprises 24,204 instances where each instance interprets the LLM's reasoning behavior using knowledge graphs (KGs) and graph attention networks (GAT), and includes explanations of LLMs such as the decoder-only Llama-3 and the encoder-only RoBERTa. XplainLLM also features a framework for generating grounded explanations and the debugger-scores for multidimensional quality analysis. Our explanations include why-choose and why-not-choose components, reason-elements, and debugger-scores that collectively illuminate the LLM's reasoning behavior. Our evaluations demonstrate XplainLLM's potential to reduce hallucinations and improve grounded explanation generation in LLMs. XplainLLM is a resource for researchers and practitioners to build trust and verify the reliability of LLM outputs.

==> main/intro.tex <==

\section{Introduction}
Large Language Models (LLMs) \citep{kenton2019bert, liu2019roberta, brown2020language, anil2023palm} have significantly influenced Natural Language Understanding (NLU) \citep{liu2021gpt, liu2023pre}, leading to performance improvements in various tasks. As these models continue to make progress, it is important to understand the rationale behind their decision-making \citep{arrieta2020explainable}. A deeper comprehension of the LLM decision-making process is crucial to fostering trust in their predictions, enabling the design of more robust and reliable AI systems for end users. 


Development of explainable AI (XAI) as an area of research has seen the emergence of a number of methods that seek to explain the decision-making processes of machine learning models. Such methods span from local explanation techniques such as LIME \citep{ribeiro2016should} and SHAP \citep{lundberg2017unified}, to global explanation strategies such as feature importance \citep{casalicchio2019visualizing}. Despite substantial progress in explaining machine learning models, these methods under-perform when deployed for LLMs, particularly in complex tasks such as question-answering (QA), making the output difficult for humans to understand. The inherent complication and lack of transparency in LLMs \citep{wu2022ai}, combined with context-rich commonsense reasoning, necessitates constructing more human-understandable and comprehensive explanations to faithfully interpret their predictions.


Current explanation methods for LLMs primarily focus on attention mechanisms \citep{clark2019does,bills2023language} and feature-based interpretations \citep{jacovi2021contrastive}. These approaches bases the explanations on self-attention weights in models like BERT \citep{kenton2019bert} and GPT-2 \citep{radford2019language}, and deduces correlations between input tokens and the model's predictions. However, the relationships highlighted in these generated explanations are difficult to understand for humans. 
%However, the highlighted relationships in the generated explanations bears little semblance to human-understandable rationales. 
Moreover, attention can be difficult to interpret due to the typically complex inter-layer interactions, and may not align the relative importance of tokens in the model's reasoning process \citep{hahn2020theoretical,sajjad2022neuron}. Feature-based explanation methods, in contrast, aim to quantify the contribution of individual features or tokens to the model output, but they fail to capture the wider context and relations that are fundamental to understanding the model's reasoning \citep{molnar2022general}. 



We introduce \datasetname{}, a dataset that addresses the growing need for transparency, explainability, and understandability in the decision-making processes of LLMs. By integrating knowledge graphs (KGs) and graph attention networks (GAT)~\citep{veličković2018graph}, our dataset provides a human-understandable explanation of LLM decision-making in QA tasks. 
We link the LLM reasoning process to the entities and relations within KGs to help provide an intuitive and interpretable representation of the LLM's decision-making process. Through the linked connections, researchers can gain deeper insights into the underlying rationale for predictions. Our process can also help facilitate model tuning, debugging, robustness evaluation and demonstration in in-context learning. \datasetname{} includes 12,102 question-answer-explanation (QAE) triples and aims to drive improvements in both the performance and explainability of LLMs. Our evaluation shows that LLMs with explanations enhance performance by an average of 2.4\% when decision-making knowledge is transferred between LLMs. LLMs with explanations outperform the benchmark, with a performance gap extending to 17\%.
The overall quality of explanations achieves an average score of 0.87/1.00 by human evaluators, and an average of 0.89/1 by automated evaluators. 


\textbf{Contributions and significance of the dataset } \; In this paper, we make several key contributions to the field of explainable AI for LLMs:
\begin{itemize}
    \item Bridging the Gap with Natural Language: To the best of our knowledge, \datasetname{} is the first dataset to capture the most influential elements behind the model reasoning and present the decision-making process through human-understandable explanations. 
    Our dataset extends beyond merely explaining the ``why''; we emphasize the ``why not'', introducing a novel paradigm in transparent AI explainability.
    \item Comprehensive Understanding of Model Reasoning: \datasetname{} incorporates \emph{reason-elements} from KGs, top-ranked \emph{reason-elements}, \emph{why-choose} and \emph{why-not-choose} explanations. The goal is to empower the community to delve deeper into the decision-making dynamics of LLMs. This work contributes to enhancing the knowledge and the transparency of LLM reasoning.
    \item Aligning Human Understanding and Model Explainability: \datasetname{} organizes the decision-influencing elements into coherent natural language sentences. Our explanations can be used in reinforcement learning from human feedback (RLHF) \citep{christiano2017deep}, to support related research. We evaluate the quality of our explanations through both automated and human evaluations, and the results underscore our dataset's quality on multiple metrics.

    
\end{itemize}



